Markovian Pandora's box

In this paper, we study the Markovian Pandora's Box Problem, where decisions are governed by both order constraints and Markovianly correlated rewards, structured within a shared directed acyclic graph. To the best of our knowledge, previous work has not incorporated Markovian dependencies in this setting. This framework is particularly relevant to applications such as data or computation driven algorithm design, where exploration of future models incurs cost. We present optimal fully adaptive strategies where the associated graph forms a forest. Under static transition, we introduce a strategy that achieves a near optimal expected payoff in multi line graphs and a 1/2 approximation in forest-structured graphs. Notably, this algorithm provides a significant speedup over the exact solution, with the improvement becoming more pronounced as the graph size increases. Our findings deepen the understanding of sequential exploration under Markovian correlations in graph-based decision-making.

==> content/ind_growth.tex <==
\subsection{Independent Growth in Model Capability}

\yy{story: gradient descent}

\begin{assumption}[Independent Growth in Model Capability]\label{assu:ind_growth}
 For each box $i \in [n]$, let the model capability be $\theta_i$. The incremental model capability is defined as $\delta_i = \theta_i - \theta_{i-1}$, where $\delta_i$ follows a distribution $\Delta_i$, and $\E[\delta]_i >0 $. For any $i \neq j \in [n]$, $\Delta_i$ and $\Delta_j$ are independent. The reward of box $i$ is:
    \begin{align*}
        R_i = f\left(\sum_{j \in [i]} \delta_j\right) = f(\theta_i),
    \end{align*}
    where $f: \mathbb{R} \to \mathbb{R}$ is a concave function, capturing diminishing returns as cumulative capability increases.
    
\end{assumption}

\subsubsection{Full Information Setting}\label{subsec:full_info}

\begin{lemma}[Full Information: Independent Growth]\label{lem:full_info_independent}
The optimal strategy for setting in Ass.~\ref{assu:ind_growth} is that, given current time $i$ and capability $\theta_i$, to search over all $j$, if there exist any $j$ such that $\E[f(\theta_j)] - \sum_{l \in [j]} c_l >0$. 
\yy{the difficulty lies in that $ f(\E[\theta_j]) >  \E[f(\theta_j)]$ for concave function. }

    
\end{lemma}

\yy{this setting seems less interesting =.= since the solution is trivial in some sense...}

